How VADER is your AI? Towards a definition of artificial intelligence systems appropriate for regulation

Artificial intelligence (AI) has driven many information and communication technology (ICT) breakthroughs. Nonetheless, the scope of ICT systems has expanded far beyond AI since the Turing test proposal. Critically, recent AI regulation proposals adopt AI definitions affecting ICT techniques, approaches, and systems that are not AI. In some cases, even works from mathematics, statistics, and engineering would be affected. Worryingly, AI misdefinitions are observed from Western societies to the Global South. In this paper, we propose a framework to score how validated as appropriately-defined for regulation (VADER) an AI definition is. Our online, publicly-available VADER framework scores the coverage of premises that should underlie AI definitions for regulation, which aim to (i) reproduce principles observed in other successful technology regulations, and (ii) include all AI techniques and approaches while excluding non-AI works. Regarding the latter, our score is based on a dataset of representative AI, non-AI ICT, and non-ICT examples. We demonstrate our contribution by reviewing the AI regulation proposals of key players, namely the United States, United Kingdom, European Union, and Brazil. Importantly, none of the proposals assessed achieve the appropriateness score, ranging from a revision need to a concrete risk to ICT systems and works from other fields.

==> appendices/premises.tex <==
\section{Premises that should underlied AI definitions for regulation}
\label{Sec:Premises}

As a concrete case study to ground our discussion, we consider the OECD 2019 and 2023 definitions~\cite{oecd2019ai,oecd2023ai}, respectively given and discussed for each premise alongside their justification. To have all premises defined, justified, and discussed in a single section, we reproduce here the justification of Premises 5--7 also given in Section~\ref{Sec:Towards}. 

\begin{quote}
An AI system is a machine-based system that can, for a given set of human-defined objectives, make predictions, recommendations, or decisions influencing real or virtual environments. AI systems are designed to operate with varying levels of autonomy.    
\end{quote}

\begin{quote}
An AI system is a machine-based system that, for explicit or implicit objectives, infers, from the input it receives, how to generate outputs such as predictions, content, recommendations, or decisions that can influence physical or virtual environments. Different AI systems vary in their levels of autonomy and adaptiveness after deployment.
\end{quote}
\setcounter{premise}{0}
\begin{premise}
\textbf{Technology agnosticity.} Definitions should not include technologies which can become obsolete in time.
\end{premise}
\noindent \textit{Justification}. The rapid evolution of ICT incurs in the proposal of novel technologies each year. As such, an AI regulation that is not agnostic will need constant revision, which may altogether compromise its effectiveness due to bureaucracy.

\noindent \textit{Discussion}. The original OECD 2019 definition is high-level enough to be agnostic to rapid technology development. The updates introduced in the OECD 2023 definition did not compromise its technology agnosticity.

\begin{premise}
\textbf{Technology neutrality.} Definitions should not be in favor or in detriment of specific sectors of the market.
\end{premise}         

\noindent \textit{Justification}. Technology regulation can affect the market when some technologies are favored in detriment of others. Collaboration with a wide range of industry sectors is required to ensure neutrality in the AI definition agreed upon.

\noindent \textit{Discussion}. The original OECD 2019 definition is high-level enough to be agnostic to rapid technology development. The updates introduced in the OECD 2023 definition did not compromise its technology neutrality.

\begin{premise}
\textbf{Technical unambiguity.} Definitions should employ only technical terms that are unambiguous.
\end{premise}

\noindent \textit{Justification}. Technology regulation poses a challenge for regulator from diverse backgrounds due to the need of precise and accurate technical terms. If ambiguous or imprecise terms are employed, the scope and implications of the regulation can be significantly affected.

\noindent \textit{Discussion}. The original OECD 2019 definition is high-level enough to be agnostic to rapid technology development. The updates introduced in the OECD 2023 definition did not compromise its technical unambiguity.

\begin{premise}
\textbf{Objectivity.} Definitions should adopt only objective terms, i.e. the rational behavior perspective~\cite{russell2020}. 
\end{premise}

\noindent \textit{Justification}. The rationale behind this premise is to avoid AI definitions that include terms that are subjective. In particular, adopting the rational behavior perspective avoids stirring a discussion on complex subjects such as intelligence, consciousness, and cognition.\sloppy

\noindent \textit{Discussion}. The original 2019 OECD definition is objectively defined in terms of the rational behavior perspective. The updates introduced in the OECD 2023 definition did not compromise its objectivity.

\begin{premise}
\textbf{Exclusion of non-ICT works.} Works such as techniques, approaches, products, and processes from non-ICT fields should be excluded from the scope of the definition.  
\end{premise}

\noindent \textit{Justification}. Two different situations motivate this premise. The first concerns definitions where a (non-)exhaustive list of techniques and approaches qualifies an AI system. Often, such a list includes the works given in Table \ref{tab:techniques}. Relevant examples are the terms (i) \textit{optimization}, which incorrectly includes all of \textit{mathematical} optimization~\cite{GilMurWri2021} instead of only \textit{heuristic} optimization~\cite{Hoos2005}, and; (ii) \textit{statistics} or \textit{statistical approaches}, which incorrectly include the statistics literature that assumes that the data are generated by a given stochastic data model instead of only the statistics literature that uses algorithmic models and treats the data mechanism as unknown~\cite{breiman2001}. The second situation concerns definitions where no list of techniques and approaches is adopted. In this case, the definition often becomes so general that it may include works from other non-ICT fields. The most straightforward examples come from engineering, where works from fields like electrical, electronic, and mechanical engineering may fit definitions incorrectly. 

\noindent \textit{Discussion}. The original 2019 OECD definition does not list techniques and approaches as an AI-system qualifier. Furthermore, the expression ``\textit{machine-based system that can (...) make (...) decisions influencing real (...) environments}'' is so broad that many engineering devices would fit this description. Examples from our validation dataset range from simple electronic devices like a thermostat to classical mechanical engineering systems, such as the steam engine governor. The updates introduced in the OECD 2023 definitions did not make the novel definition compliant with this premise, as it includes the equivalent expression ``\textit{system that (...) infers (...) how to generate outputs such as (...) decisions (...) influencing physical (...) environments}''.

\begin{premise}
\textbf{Exclusion of non-AI ICT techniques, approaches, and systems.} Techniques and approaches from ICT disciplines other than AI should be excluded, as well as systems that do not employ AI techniques and approaches.
\end{premise}

\noindent \textit{Justification}. The two different scenarios that motivated the previous premise also motivate this premise. In detail, (non-)exhaustive list of techniques and approaches that qualify an AI system often adopt terms that are too broad, including techniques and approaches that originate in an ICT discipline other than AI. A relevant example is search, which incorrectly includes uninformed techniques that originate in the \textit{algorithms} and \textit{complexity} ICT discipline \cite{Cormen2022}. In turn, when no list is provided, broad definitions may erroneously include ICT systems that in no way make use of AI techniques and approaches. One relevant example is to refer to AI systems as systems that are employed to assist in decision-making, which not necessarily are AI systems.

\noindent \textit{Discussion}. As previously mentioned, the original 2019 OECD definition does not include an AI-system qualifier list of techniques and approaches. In addition, the expression ``\textit{system that can (...) make (...) recommendations (...) influencing real (...) environments}'' is broad enough that many ICT systems employed to assist decision-making would qualify. Examples from our validation dataset include enterprise resource planning systems, as well as business intelligence dashboards. The updates introduced in the OECD 2023 definitions did not make the novel definition compliant with this premise, as it includes the equivalent expression ``\textit{system that (...) infers (...) how to generate outputs such as (...) recommendations (...) influencing physical (...) environments}''.

\begin{premise}
\textbf{Inclusion of all AI techniques and approaches.} All techniques and approaches that can qualify a system as AI should be included.
\end{premise}

\noindent \textit{Justification}. The two different scenarios that motivated the previous premises also motivate this premise.  In detail, (non-)exhaustive list of techniques and approaches that qualify an AI system sometimes oversee AI techniques and approaches. One example is overly focusing on learning and missing out on other aspects of AI, such as search and reasoning. In turn, when no list is provided, broad definitions can very easily defined AI systems in a way that only accounts for a subset of techniques and approaches.

\noindent \textit{Discussion}. As previously mentioned, the original 2019 OECD definition does not include an AI-system qualifier list of techniques and approaches. In addition, the expression ``\textit{system that can (...) make predictions, recommendations, or decisions influencing real (...) environments}'' misses out on generative AI. The updates introduced in the OECD 2023 definitions made the novel definition compliant with this premise, as the definition now reads ``\textit{system that (...) infers (...) how to generate outputs such as predictions, content, recommendations, or decisions that can influence physical or virtual environments}''.
